Assessing the Cost of Network Simplifications in Long-Term Hydrothermal Dispatch Planning Models

The sustainable utilization of hydro energy relies on accurate estimates of the opportunity cost of the water. This value is calculated through long-term hydrothermal dispatch problems (LTHDP), and the recent literature has raised awareness about the consequences of modeling simplifications in these problems. The inaccurate representation of Kirchhoff's voltage law under the premise of a DC power flow is an example. Under a non-linear AC model, however, the LTHDP becomes intractable, and the literature lacks an accurate evaluation method of different modeling alternatives. In this paper, we extend the state-of-the-art cost-assessment framework of network approximations for LTHDP and bring relevant and practical new insights. First, we increase the quality of the assessment by using an AC power flow to simulate and compare the performance of five policies based on different network approximations. Second, we find that the tightest network relaxation (based on semidefinite programming) is not the one exhibiting the best performance. Results show that the DC {power flow} with quadratic losses approximation exhibits the lowest expected cost and inconsistency gaps. Finally, its computational burden is lower than that exhibited by the semidefinite relaxation, whereas market distortions are significantly reduced in comparison to previously published benchmarks based on DC power flow.

==> Sec-Cases.tex <==
In this section, the quality of the five approximations for the network constraints under study are compared. The time inconsistency gap and other relevant operative indexes such as reservoir levels, thermal generation, and spot prices are studied to provide a more in-depth understanding of their differences. 

The inconsistent policies will be denoted according to the pair of network models used in the planning and implementation phases. In this work, all policies are evaluated under the same basis, with the most accurate network formulation in the implementation model, the AC power-flow model \eqref{AC_W_PF}, using the same set of out-of-sample scenarios (scenarios not used in the planning stage where the cost-to-go functions were estimated). Thus, for instance, the policy used in the planning phase of the transportation NFA model is named \textbf{NFA-AC inconsistent policy}. Analogously, the other policies will be named: \textbf{SOC-AC inconsistent policy}, \textbf{SDP-AC inconsistent policy}, \textbf{DC-AC inconsistent policy}, and \textbf{DCLL-AC inconsistent policy}. Finally, to estimate the time-inconsistency gap, we will also assess the cost for the planning policies, namely, \textbf{NFA planning policy}, \textbf{SOC planning policy}, \textbf{SDP planning policy}, the \textbf{DC planning policy}, and \textbf{DCLL planning policy}, each of which relies solely on their respective relaxations for both planning and implementation. 

\subsection{Three-bus test system with loop}

As a case study, we use the three-bus system from \cite{7859406} to illustrate the effects of the underlying policies. A definition of case parameters following our notation can be found in \cite{AndrewThesis}. All three buses are connected in a loop. One hydro unit is located at bus $1$, one thermometric unit at bus $2$, and the most expensive thermoelectric unit and the demand at bus $3$.


Table \ref{table_costs_case3} shows the following information in its five columns: names of the inconsistent policies; the expected cost of the planning policies; the expected cost of the inconsistent policies at the implementation step (with the out-of-sample scenarios and AC power flow); the time-inconsistency GAP (the difference between the implementation and planning costs); and finally, the total computing times took for converging the SDDP with each network approximation (which is a measure of the computational burden that would be faced by system operators opting a given network representation).
%
\begin{table}[!ht]
% increase table row spacing, adjust to taste
\small
\renewcommand{\arraystretch}{1.3}
\centering
\caption{3-Bus Case: Planning and Implementation Policy Comparison.}
\label{table_costs_case3}
\begin{tabular}{c c c c c}
\hline
 \multicolumn{1}{p{0cm}}{\centering Policy \\ (plan,imp)} & \multicolumn{1}{p{0cm}}{\centering Planning \\ ($10^6 \$$)} & \multicolumn{1}{p{2cm}}{\centering Implementation \\ ($10^6 \$$)} & \multicolumn{1}{p{0cm}}{\centering GAP \\ (\%)} & \multicolumn{1}{p{0cm}}{\centering Time \\ (min.)} \\
\hline 
NFA-AC & $43.2317$ & $54.7234$ & $26.4$  & $5.40$\\
SOC-AC & $45.0477$ & $54.9197$ & $21.7$  & $23.92$\\
SDP-AC & $45.4524$ & $48.2853$  & $6.1$  & $47.47$\\
DC-AC & $43.3940$ & $48.8891$  & $12.5$  & $5.41$\\
DCLL-AC & $45.4158$ & $48.0700$ & $5.68$  & $16.09$\\
\hline
\end{tabular}
\end{table}


The first important remark from Table \ref{table_costs_case3} is that the GAP increases with the simplification (relaxation) level. This indicates that the more optimistic one is in the planning phase, the higher will be the expected regret, i.e., the deviation of the implementation cost with regard to the planning one.
%Note that as DC-based policies are not relaxations.
%of neither the SOC nor the SDP based policies.
The inclusion relation between relaxations are the following: NFA is a relaxation of all the others, SOC is a relaxation of the SDP, and DC is a relaxation of the DCLL. 

The NFA-AC inconsistent policy, the simplest planning model, also features the lowest time, which is the main reason why the NFA simplification is widely adopted in practical studies \cite{maceiral2018twenty}. This simplification induces high operative costs in the implementation phase when an AC power flow is used to simulate the policy. 

The SOC-AC inconsistent policy features the second-highest GAP. Despite convex, this formulation is not easy to solve having the second higher computing time. This 3-Bus case is fully connected, hence it is one of the worst types of network for the SOC relaxation, opposed to radial systems \cite{1664986}. Interestingly, the SOC-AC policy performs slightly worse than the NFA-AC policy in the implementation phase, despite having a higher cost at the planning phase.
%The examination of the cost-to-go functions can explain this. Despite the difference between the cost-to-go functions produced by the NFA and SOC models (Figure \ref{fig:exp_case3} (c)), due to the cost of losses not represented in the NFA model, the NFA model leads to slightly lower derivatives. Consequently, SOC produces slightly higher hydro opportunity costs for the implementation model.
%This explains the lower cost of the NFA-AC policy in comparison to the SOC-AC in the implementation phase.
This suggests that the SOC approximation might exhibit inferior performances in the presence of very meshed grids. 

The SDP-AC inconsistent policy has the tightest convex relaxation and the second-lowest GAP and cost in the implementation phase. Also, the implementation cost is almost equal to the lowest implementation cost (DCLL-AC). This benefit comes with the cost of the highest computational burden. %As will be further shown, this model proves to be the most coherent and consistent in terms of operating results.

The {DC-AC inconsistent policy} performs better than the SOC-AC and worse than the SDP-AC in terms of expected implementation cost. Moreover, it is a competitive policy having a GAP less than $2\%$ higher than the DCLL-AC policy. Although it does not model transmission losses,
%as per Figure \ref{fig:FCF_and_deriv_case3} (b), 
it is capable of capturing the relevant operative constraints imposed by KVL and obtaining opportunity costs similar to those of the SDP model, but faster. %This model is competitive and can be seen as an alternative to the conic formulations in the presence of meshed systems with low loss levels. 

The {DCLL-AC inconsistent policy} results indicate the best performance in terms of implementation cost, GAP, and average computing times for a small system. It puts together the DC model's capability to approximate KVL constraints and a reasonable description of the transmission losses. These results demonstrate a quadratic approximation can perform better than the conic SDP relaxation. Additionally, DCLL is more than two times faster than SDP, thereby representing an interesting alternative in the presence of meshed grids with non-negligible losses. 

To further analyze these results, the expected storage is depicted in Figure \ref{fig:exp_case3} (a)
and the expected spot prices in Figure \ref{fig:exp_case3} (b) for all analyzed policies. %This analysis is done in light of what we observed in the cost-to-go functions in Figure \ref{fig:exp_case3} (c). %The solid lines in this figure represent the cost-to-go function on the points . The dotted lines are the output of the simulation of the inconsistent policies under the out-of-sample scenarios. 
In Figure \ref{fig:exp_case3} (a), notice that the {NFA planning policy} is the most optimistic (relaxed) model, leading to an aggressive use of the water that can not be implemented in practice due to the KVL constraints. This produces the highest inconsistency gap between the planning and the implemented policies depicted in both reservoir levels and spot prices. Conversely, the SOC model depicts an apparently consistent policy in terms of reservoir level. However, this relaxation precisely affects the KVL representation in the model, by further relaxing (2.a) dropping the semidefinite parcel of this constraint. Hence, in the presence of cycles, this model also exhibits a myopic view of KVL constraints, driving the system to extremely low expected reservoirs levels as the NFA does. Hence, based on these two relaxations, the system operator, without acknowledging the electric constraints in the future, exposes the system to dangerous operating points and infeasible dispatches (requiring load curtailment). These infeasibilities cause a huge increase in the average spot prices as shown in Figure \ref{fig:exp_case3} (b). This relevant market distortion in spot prices, which is also accompanied by similar distortions in thermal generation, highlights the risk of ignoring KVL constraints in the planning stage.

%In Figure \ref{fig:exp_case3} (c), w
In contrast to the aforementioned formulations ignoring the KVL constraints, there are the DC, SDP, and DCLL models. All of them consider approximations of the KVL constraints, thereby being aware of the operative difficulties of future stages caused by this constraints. Consequently, in the planning stage, their policies value the water accordingly, saving significantly more water than the KVL-myopic policies (NFA and SOC) as shown in \ref{fig:exp_case3} (a). This better representation of systems' constraints drives the reservoirs to safer levels enabling the system operator to circumvent the discrepancies between the planning and implementation models. As a consequence, spot prices distortions are significantly mitigated. The {DCLL planning policy} is even more pessimistic than the SDP and stores more water than the DC model. Still, the more accurate representation of the SDP relaxation allows a more efficient use of the stored water, leading to even lower discrepancies between planned and implemented spot prices.


\begin{figure*}[htb]
\centerline{\includegraphics[width=0.9\linewidth]{Figures/exp_case3.png}}
\caption{Three-bus case: (a) Expected Reservoir levels, (b) expected spot prices}
%, and (c) second-stage approximated cost-to-go functions.
\label{fig:exp_case3}
\end{figure*}

According to Figure \ref{fig:exp_case3} (b), significant structural differences are found in the average spot prices between the respective planning and implementation policies. This stems from the fact that additional and expensive dispatches are needed to compensate for the optimistic view of the approximations in critical states (low reservoir levels). In the same Figure \ref{fig:exp_case3} (b), the {NFA planning policy} presents the lowest prices, as expected for the most relaxed problem that uses water resources as if no electrical constraints exist. The {SOC planning policy} has the second-lowest price given that it does not provide accurate representations of the network in the presence of cycles. In the sequel, the {DC planning policy}, {SDP planning policy}, and {DCLL planning policy} still provide a simplified version of the true network, albeit their representation are capable of considerably reducing the spot-price spikes. These better behaved spot-price profiles stem from the better representation of the electrical constraints, which, although more expensive in the planning phase, allows the system to achieve better states in the implementation phase. Furthermore, the more inconsistent is the policy, the higher are the spot-price spikes. This can be seen by comparing the {SDP-AC inconsistent policy}, the {SOC-AC inconsistent policy}, and the {NFA-AC inconsistent policy} which, in this order, incrementally relax the electric constraints in the planning stage. Notice that the {SOC planning policy} and the {SOC-AC inconsistent policy} differ here since the electrical operation provided by the planning policy is infeasible even though it has found an implementable storage management schedule on average. 

\subsection{28-bus case study}

In order to further analyze the impacts of time inconsistency due to network formulations, we now use a larger case study using realistic data from the Bolivian system with the following characteristics: 28 buses, 26 loads, 34 generators (11 hydro generators), and 31 branches. The system is mostly radial with only 3 cycles. 


\begin{table}[!ht]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
\centering
\caption{28-bus case: Planning and Implementation Policy Comparison.}
\label{table_costs_bolivia}
\begin{tabular}{c c c c c}
\hline
 \multicolumn{1}{p{0cm}}{\centering Policy \\ (plan,imp)} & \multicolumn{1}{p{0cm}}{\centering Planning \\ ($10^6 \$$)} & \multicolumn{1}{p{2cm}}{\centering Implementation \\ ($10^6 \$$)} & \multicolumn{1}{p{0cm}}{\centering GAP \\ (\%)} & \multicolumn{1}{p{0cm}}{\centering Time \\ (min.)} \\
\hline  
NFA-AC & $0.58687$ & $0.68735$ & $17.067$ & $4.67$ \\
SOC-AC & $0.60818$ & $0.60935$ & $0.193$ & $119.23$ \\
DC-AC & $0.58714$ & $0.64523$ & $9.855$ & $5.22$ \\
DCLL-AC & $0.61310$ & $0.60941$ & $-0.602$ & $54.33$ \\
\hline
\end{tabular}
\end{table}

The {NFA-AC inconsistent policy} is still responsible for the higher expected cost in the implementation step when evaluated with the AC power flow. This table shows that the SOC convex relaxation produces a very small inconsistency GAP and one of the lowest operating costs. Under mild conditions, this relaxation is tight for radial systems (\cite{1664986}). Thus, for the specific cases where cycles do not constraint much the least cost dispatch, which is the case of this study, this relaxation performs reasonably well in terms of cost (policy quality). Nevertheless, this relaxation imposes the highest computational burden. It is worth mentioning that the SDP formulation has shown to be intractable for this problem and the hardware available. Therefore, SDP-based policies' tractability poses a clear obstacle for the practical use of this network model even for medium-sized systems.

The {DC-AC inconsistent policy} performed better than the NFA-AC and worse than the {SOC-AC inconsistent policy} in terms of GAP and expected implementation cost. It also exhibits a significantly lower computational burden than the SOC relaxation and performance close to NFA. Thus, the DC network model provides an acceptable choice for practical applications with medium-sized systems. On the other hand, the {DCLL-AC inconsistent policy} features a statistically indistinguishable cost difference with the implementation policy based on the SOC relaxation (significance level of 0.05). Therefore, although the DCLL features a higher computational burden than the DC, it exhibits high quality solutions, the lowest inconsistency GAP, and a lower computational burden than the SOC relaxation (two times faster). It puts together the DC model capability of approximating KVL constraints and a reasonable description of the transmission losses. These results demonstrate a quadratic approximation can have a close performance to the nonlinear SOC relaxation even in approximately radial systems.

% when this study was conducted.

To further analyze these results, the expected thermal generation is depicted in Figure \ref{fig:exp_bolivia} (a) and the expected spot prices in Figure \ref{fig:exp_bolivia} (b) for all analyzed policies. For NFA and DC, we see high thermal dispatches when evaluated under a AC power flow ({NFA-AC inconsistent policy} and {DC-AC inconsistent policy}) in Figure \ref{fig:exp_bolivia} (a) and, thus, also higher nodal prices are induced as seen in Figure \ref{fig:exp_bolivia} (b). SOC and DCLL formulations present sufficiently good electric constraints approximations and sufficiently good power flow loss approximations for the low loss system without significant cycles in this case. Therefore, their planned and implemented dispatches are very close to each other, mitigating the market distortions observed for the NFA and DC-based policies.

\begin{figure*}[htb]
\centerline{\includegraphics[width=0.9\linewidth]{Figures/exp_bolivia_2.png}}
\caption{Case28: (a) Expected Thermal Generation; and (b) Expected Spot Price levels with time inconsistency due to simplifications in
transmission-line modeling.}
\label{fig:exp_bolivia}
\end{figure*}


==> Sec-Conclusion.tex <==

In this work, we estimate and analyze the cost and impact of network simplifications in hydrothermal operation planning problems. We extend the results of \cite{7859406} by extending the long-term hydrothermal operation planning problem to consider five different network formulations through a novel open-source package \textit{HydroPowerModels.jl}. The framework allows estimating policies optimized with simplified network formulations and evaluating their quality with the more constrained and realistic AC network model. Results shows that the optimistic assessments of the water value induce high dispatch costs and market distortions such as high and unexpected spot-price spikes and thermoelectric dispatches. In this paper we further identified the risk of poorly approximating the KVL constraints in the planning stage (when the opportunity cost of the water is calculated).

In light of the results from the case studies, we can draw conclusions for each model. 
The \textbf{Network Flow Approximation} presents, on average, the lowest computational burden. However, this comes with the cost of exposing the system operator to high regrets due to the null representation of KVL constraints and losses. As a result, we find high operational costs in the actually implemented dispatches (frequently related to expensive and polluting thermal resources), and unjustified volatile spot-price profiles. The \textbf{Second Order Cone relaxation} also provides poor approximations of the Kirchhoff's Voltage Law. Therefore, in the presence of cycles, this model also exhibits the typical distortions in spot prices and thermal generation dispatches. Its computational burden is higher than linear formulations, but significantly lower than the semidefinite relaxation. 

The \textbf{Semidefinite relaxation} exhibits low inconsistency levels in the presence of cycles and consequently low distortions in both prices and thermal generation dispatches. However, this benefit comes with a high computational burden, which prevents its application in larger cases.
The \textbf{DC approximation} is a standard and fair approach, performing reasonably well (small gap and low distortions in prices and dispatches) in all instances and with a reduced computational burden. Interestingly, the \textbf{DC with line losses approximation} has the best performance in terms of implementation cost, and it consistently presents the smallest inconsistency gaps, very low distortions in prices and dispatches in comparison to the alternatives. The computational burden is not as reduced as in the DC case, as it is based on quadratic (convex) programming, but it is still faster than the two convex conic relaxations. Consequently, this approximation appears as a relevant alternative for the harder to solve conic relaxations and can bring significant benefits compared to the widely used Network Flow Approximation model currently adopted in Brazil. 

%Acknowledging the challenges of introducing quadratic models in the SDDP for realistic network dimensions, we highlight as a relevant research topic the study of new approximation methods capable of capturing the joint effect of line losses and Kirchhoff's Voltage Law and specialized decomposition algorithms for the resulting quadratic DC with line losses problem.


==> Sec-Introduction.tex <==
\IEEEPARstart{A}{ssessing} the value of systems' scarce resources is a key activity of power system operators, especially those in charge of hydrothermal power systems \cite{pereira1991multi}. Such assessment aims at evaluating implicit opportunity costs of relevant systems' resources, such as water, which can be stored and used in future periods to prevent the expensive thermal generation or load shedding. Due to its fast response, hydroelectric power plants also play a crucial role in paving the way for the integration of other renewable sources such as wind and solar. Besides that, hydropower is still today one of the most relevant renewable resources in the world \cite{EIA2019}. Therefore, clearly, an accurate assessment of the water opportunity cost is crucial for practical purposes, as highlighted in \cite{street2020assessing}.

Opportunity costs of systems' relevant resources, such as water in hydrothermal dispatch (HTD), are generally estimated through long-term operational planning studies in the form of multistage stochastic linear models \cite{pereira1991multi}. The state-of-the-art solution method for such large-scale optimization problems is the so-called Stochastic Dual Dynamic Programming (SDDP) proposed in \cite{pereira1991multi}. The SDDP algorithm iteratively approximates the future cost of operation, also known as the cost-to-go function, as a piecewise linear convex function of the amount of water stored in the reservoirs. The computational efficiency of SDDP notwithstanding, the algorithm relies on strong assumptions such as convexity of the dispatch problem defining the cost-to-go function. This is a constant limitation in the vast part of the literature on the subject (we refer to \cite{Helseth2016}, where an agent sells reserve capacity in a competitive market, and \cite{Street2017}, where the $n-K$ security criterion is incorporated within the centralized cost minimization framework). More recently, however, an interesting extension to consider binary variables (considering a non-convex subproblem), the SDDiP was proposed in \cite{Zou2019} and applied in \cite{Martin2019}.  

Despite the recent advances in the SDDP technique, given the scale long-term hydrothermal planning studies, modeling simplifications are always needed by virtue of computational tractability of the resulting multistage stochastic programming problem. However, the operative policy is usually implemented by a more detailed short-term model coupled with the opportunity cost assessment of the simplified long-term operation planning model. Consequently, the implemented operative decisions may significantly differ from the planned ones even if the same scenario takes place, and the implementation model differs from the planning model solely on one feature such as the network model \cite{7859406}. Such inconsistency can be understood as a model-misspecification risk. As demonstrated in \cite{7859406}, statistically significant time-inconsistency gaps can be induced when the Kirchhoff's Voltage Law (KVL) and the $n-1$ security criterion are disregarded under the DC power flow approximation. In \cite{street2020assessing}, statistically significant gaps are found due to the hazard-decision simplification, where the information-revelation process of the inflow uncertainty is simplified by a one-step-ahead anticipative model.

The studies in \cite{7859406} assume a DC power flow model as the reference model for the assessment of the time-inconsistency gap when planning the system operation using the transportation network flow approximation model (NFA). However, as reported in the technical literature (see \cite{low2014convex} and \cite{dvijotham2016error}), DC power flow approximation still produces significant discrepancies and the actual operation is better represented by an AC power flow model. Thus, in this work, we extend previously reported results on the impact of network simplifications on two fronts: 1) the more accurate AC power-flow model is considered as the reference model in the inconsistency gap and market distortion assessments, and 2) five network modeling simplifications largely used in the literature are considered in our comparison. These extensions allow us to identify the pros and cons of different network models in terms of their approximation quality and computational burden. 

To achieve the aforementioned goals 1) and 2), reliable and flexible implementations of the SDDP algorithm allowing multiple power flow approximations are needed. Unfortunately, such a tool was not available. Therefore, an open-source SDDP tool with this feature, \textit{HydroPowerModels}, was developed and made available \cite{Rosemberg2020}. This tool enables not only the assessment of the results found in this work but also allows researchers in the electrical industry to test new ideas, leveraging state-of-the-art solution methods and mathematical formulations for the HTD. 

The objective of this work is to present an open-source computational framework
% , comprising a methodology and an open-source computational package, 
for testing the operative and economic impact of modeling simplifications over the network power-flow in hydrothermal power systems. Among the myriad of formulations available in the package, 
we focused on assessing the cost and operative performance of the following model approximations: NFA, currently in use by the Brazilian system operator \cite{7859406}; the second-order cone relaxation (SOC) \cite{1664986}; the semidefinite programming relaxation (SDP) \cite{6345272}; the DC power-flow approximation (DC) \cite{Stott2009_DC}, and the DC with line-loss power-flow approximation (DCLL) \cite{dcll_coffrin}. All the previously mentioned formulations are tested as approximations for the network model in the planning stage of the HTD, where the cost-to-go function is built through the SDDP algorithm. Then, we evaluate each approximation by simulating the system's operation, which minimizes costs under AC power-flow constraints (see \cite{carpentier1962contribution} and \cite{Cain2012}). 

In this context, the main contributions of this work are twofold:

\begin{enumerate}
    
    \item The extension of the results of \cite{7859406} comparing the performance of five network formulations, namely, NFA, SOC, SDP, DC, and DCLL under a more accurate implementation model using the AC power-flow formulation. With this computational framework, we can analyze and compare the results of the different planning policies using different network simplifications and measure the tradeoff between computational burden and solution quality.
    
    \item To study the detrimental effect of network simplifications while identifying the tradeoff between the computational burden and solution quality for each network model. More specifically, we show that the SOC approximation induces a planning policy with poor performance and dispatch distortion when the system is fully meshed and with good performance when the system is fully radial. Under mild conditions, this is always obtained with a reasonable computational burden. The planning policy based on the SDP relaxation has a low inconsistency gap but comes with a high computational burden. The DC-based planning policy performs reasonably well (but worst than SDP) with low distortions in prices and thermometric dispatches in all instances and with a reduced computational burden. Finally, the DCLL approximation exhibits the lowest system cost when evaluated with the full AC model, the lowest inconsistency gap, and its computational burden is lower than that presented by the convex conic relaxations (SOC and SDP). Thus, we find this modeling approximation, based on quadratic (convex) programming, as an interesting and effective alternative to reduce market distortions at a reasonable computational burden.  % conclusao ?

    % \item An open-source tool for solving hydrothermal economic dispatch problems with stochastic dynamic programming, namely \textit{HydroPowerModels} \cite{Rosemberg2020}. Programmed as a package for the Julia language, it takes advantage of the productivity and speed that this language has to stimulate collaboration and relevance. The package provides an easy-to-use framework where the user is free to choose from a variety of network formulations and study parameters. Moreover, it allows the construction of shared database of cases, helping discussions about solution methods and study choices. 
    
\end{enumerate}


The remainder of this work is organized as follows. Section \ref{sec:tb} presents the theoretical background for HTD and time-inconsistency. Section \ref{sec:pf} explains the five network approximation models derived from the AC power-flow model and presents the open-source tool to support studies of HTD. Section \ref{sec:cases} presents case studies. Relevant conclusions are drawn in Section \ref{sec:conclusion}.
 

==> Sec-Nomenclature.tex <==
\subsection*{Sets and Indices}

\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$MMM$}]
\item[$t$] Subscript to represent period $t$.
%\end{IEEEdescription}

%\subsection*{Sets and Indices}

%\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$MMM$}]
	\item[$\mathcal{N}$] Set of bus indices $n$ or $m$.
	\item[$\mathcal{N}_0$] Singleton containing reference bus index $n$ or $m$.
	\item[$\mathcal{N}_n$] Set of buses connected to bus $n$.
	\item[$\mathcal{L}$] Set of directed branches, pairs of buses $(n,m)$, where $n > m$, i.e., pairs are ordered and appear at most once.
% 	\item[$\mathcal{L}_n^+, \mathcal{L}_n^-$] Set of transmission lines/branches with destination and origin at bus $n$, respectively.
	\item[$\mathcal{I}, \mathcal{I}_n$] Set of thermoelectric units $i$ and subset  at bus $n$.
	\item[$\mathcal{H}, \mathcal{H}_n$] Set of hydroelectric units $j$ and subset at bus $n$.
	\item[$\mathcal{H}^U_j$] Set of upstream hydroelectric units $k$ to unit $j$.%, respectively.
\end{IEEEdescription}

\subsection*{Constants}

\newdimen\origiwspc%
\newdimen\origiwstr%
\origiwspc=\fontdimen2\font% original inter word space
\origiwstr=\fontdimen3\font% original inter word stretch

\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$MMM$}]
    \item[$P_{it}$, $Q_{it}$] Real and reactive power bound at generator $i$.
    \item[$C_{it}$] Cost of generator $i$.
    \item[$\overline{V}_{nt}$, $\underline{V}_{nt}$] Upper/lower magnitude voltage limits at bus $n$.
    \item[$D_{nt}$,$C^{\delta}_{nt}$] Real power load and deficit cost at bus $n$.
    \item[$Y^s_{nt}$, $Y^{sq}_{nt}$] Shunt real and imaginary admittance at bus $n$.
    %\item[$C^{\delta}_{nt}$] Deficit linear cost at bus $n$.
    \item[$G^c_{(n,m)t}$] Real part of pi-section parameters at branch $(n,m)$.
    \item[$B^c_{(n,m)t}$] Imaginary part of pi-section parameters at branch $(n,m)$.
    \item[$F_{(n,m)t}$] Apparent power limit at branch $(n,m)$.
    \item[$R_{(n,m)t}$] Resistance at branch $(n,m)$.
    \item[$X_{(n,m)t}$] Reactance at branch $(n,m)$.
    %\item[$\overline{\Delta}^{\theta}_{(n,m)t}$] Voltage angle upper bound at branch $(n,m)$.
    %\item[$\underline{\Delta}^{\theta}_{(n,m)t}$] Voltage angle lower bound at branch $(n,m)$.
    \item[$\overline{\nu}_{jt}$] Volume limit at hydroelectric units $j$.
    \item[${\nu}_{jt-1}$] Initial volume at hydroelectric units $j$.
    \item[$A_{jt}$] Possible inflows at hydroelectric units $j$.
    \item[$U_{jt}$] Outflow limit at hydroelectric units $j$.
    \item[$\rho_{jt}$] Production factor at hydroelectric units $j$.
    %\item[$C^{s}_{jt}$]  Spillage linear cost at hydroelectric units $j$.
\end{IEEEdescription}



\subsection*{Decision Variables}

\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$MMM$}]
    \item[$p_{it}$, $q_{it}$] Real and reactive power dispatch at generator $i$.
    \item[$v_{nt}$, $\theta_{nt}$] Complex voltage and Phase angle at bus $n$.
    %\item[$\theta_{nt}$] Phase angle at bus $n$.
    \item[$\delta_{nt}$, $\ell_{nt}$] Real power deficit and Loss at bus $n$.
    %\item[$\ell^{(sh)}_{nt}$] Shunt loss at bus $n$.
    \item[$u_{jt}$, $s_{jt}$] Outflow and Spillage at hydroelectric units $j$.
    \item[$\nu_{jt}$] Volume at hydroelectric units $j$.
    %\item[$s_{jt}$] Spillage at hydroelectric units $j$.
    \item[$f_{(n,m)t}$] Real power flow at branch $(n,m)$.
    \item[$f^q_{(n,m)t}$] Reactive power flow at branch $(n,m)$.
\end{IEEEdescription}

\subsection*{Operators}

\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$MMM$}]
	%\item[$\Im$] Imaginary unit.
	\item[$(\cdot)^{*}$] Complex conjugate.
	\item[$\angle(\cdot)$, $|\cdot|$] Angle and magnitude of a complex number.
	%\item[$|\cdot|$] Absolute value.
\end{IEEEdescription}

==> Sec-PFramework.tex <==

The network constraints set $\mathcal{X}_t$ can assume many forms. We present a non-standard description of power flow constraints that is key to contrast and compare the different formulations considered in this work. 
We start with the most detailed network model, the non-linear AC formulation, which will be used as the evaluation model to evaluate the quality of all subsequent formulations. In this case, the network model is the following:

$\mathcal{X}_{AC,t}$ $=$ \Big\{ $p_t, f_t, u_t, s_t, \nu_t, \delta_t, \ell_t \, $\Big\vert$ \, \exists \; q_t,v_t,\mathbf{W}_t,f^q_t$ :
\begin{subequations} \label{AC_W_PF}
    \begin{align}
        %
        & \mathrm{w}_{nmt} = v_{nt}v_{mt}  \;\; \forall(n,m) \in \mathcal{L} \label{eq_ac_w}\\
        %& \mathbf{W}_t \succeq 0 \label{eq_sdp_w}\\
        %& |\mathrm{w}_{nmt}|^2 \leq  \mathrm{w}_{nnt}\mathrm{w}_{mmt} \;\; \forall(n,m) \in \mathcal{L} \label{eq_soc_w}\\
        & \underline{V}_{nt}^2 \leq \mathrm{w}_{nnt} \leq \overline{V}_{nt}^2 \;\; \forall n \in \mathcal{N} \label{eq_voltage_acw_bounds}\\
        & (f_{(n,m)t})^2 + (f^q_{(n,m)t})^2 \leq F_{(n,m)t}^2 \;\; \forall (n,m) \in \mathcal{L} \label{eq_thermal_limit_acw} \\
        % & \underline{\Delta}^{\theta}_{(n,m)t} \leq \angle (\mathrm{w}_{nmt}) \leq \overline{\Delta}^{\theta}_{(n,m)t} \;\; \forall (n,m) \in \mathcal{L} \label{eq_angle_difference_acw}  \\
        & \sum_{\substack{i \in I_n}} q_{it} - Y^{sq}_{nt} \mathrm{w}_{nnt} -\sum_{\substack{m\in \mathcal{N}_n}} f^q_{(n,m)t} = 0 \;\; \forall n\in \mathcal{N} \label{eq_kcl_shunt_q_acw} \\
        & \ell_{nt} = Y^{s}_{nt} \mathrm{w}_{nnt} \;\; \forall n \in \mathcal{N} \label{eq_loss_acw}\\      
        & f_{(n,m)t} = \left( G_{(n,m)t} + G_{(n,m)t}^c \right) \mathrm{w}_{nnt} + \nonumber \\
        &  \left(-G_{(n,m)t} + B_{(n,m)t}\right) \mathrm{w}_{nmt}^{\Re} + \nonumber \\
        &  \left(-B_{(n,m)t}-G_{(n,m)t}\right) \mathrm{w}_{nmt}^{\Im}  \;\;  \forall (n,m)\in \mathcal{L} \label{eq_power_acw}\\
        & f_{(m,n)t} = \left( G_{(m,n)t} + G_{(m,n)t}^c \right) \mathrm{w}_{mmt} +  \nonumber \\
        & \left(-G_{(m,n)t} + B_{(m,n)t}\right) \mathrm{w}_{mnt}^{\Re} \nonumber \\
        & \left(-B_{(m,n)t}-G_{(n,m)t}\right) \mathrm{w}_{mnt}^{\Im}  \;\;  \forall (n,m)\in \mathcal{L} \label{eq_power_acw_2}\\
        & f_{(n,m)t}^q = -\left( B_{(n,m)t} + B_{(n,m)t}^c\right) \mathrm{w}_{nnt} - \nonumber \\
        &  \left(-G_{(n,m)t} - B_{(n,m)t}\right) \mathrm{w}_{nmt}^{\Re} + \nonumber \\
        &  \left(B_{(n,m)t}-G_{(n,m)t}\right) \mathrm{w}_{nmt}^{\Im}   \;\;  \forall (n,m)\in \mathcal{L} \label{eq_power_acw_q} \\
        & f_{(m,n)t}^q = -\left( B_{(m,n)t} + B_{(m,n)t}^c\right) \mathrm{w}_{mmt} - \nonumber\\
        & \left(-G_{(m,n)t} - B_{(m,n)t}\right) \mathrm{w}_{mnt}^{\Re} + \nonumber\\
        & \left(B_{(m,n)t}-G_{(m,n)t}\right) \mathrm{w}_{mnt}^{\Im}   \;\;  \forall (n,m)\in \mathcal{L} \label{eq_power_acw_q_2}\\
        & -Q_{it} \leq q_{it} \leq Q_{it} \;\; \forall i \in I \Big\},\label{eq_gen_q_bounds_acw}
    \end{align}
\end{subequations}
where $\mathrm{w}_{nmt}^{\Re}$ represents the real part of the $\mathrm{w}_{nmt}$ variable, and, $\mathrm{w}_{nmt}^{\Im}$, the imaginary part.

This formulation is actually an equivalent model to the more classical formulation \cite{carpentier1962contribution} developed in the attempt to provide better relaxations, \cite{BAI2008383,1664986,coffrin2015qc}. It uses an auxiliary variable $\mathrm{w}_{nm}$ to represent the product of the voltage from buses $n$ and $m$, i.e., $ \mathrm{w}_{nmt} = v_{nt}v_{mt}$.

In this model, the magnitude of the complex voltage is bounded in constraint \eqref{eq_voltage_acw_bounds}. 
% Angle differences between buses are bounded in \eqref{eq_angle_difference_acw}.
%
The branch complex power flow is formulated in \eqref{eq_power_acw}, to \eqref{eq_power_acw_q_2}, that are dependent on the voltage at each end of a branch. 
Note that problem induced by \eqref{AC_W_PF}, that is when $\mathcal{X}_t \leftarrow \mathcal{X}_{AC,t}$ in \eqref{OPF}, better represents reality, but is a non-linear and non-convex optimization problem. 

The AC-OPF model is a non-convex non-linear problem (NLP), not suitable for the classical SDDP algorithm. Thus, as in many applications, convex approximations and relaxations can be used to meet the SDDP convexity hypothesis \cite{molzahn2019survey}. 
In general, those formulations are simplifications of the full AC model, and each one of them focuses on some particularities of the original problem. As a result, it is relevant to understand the tradeoff between each approximation quality and model tractability.

\textit{Relaxations} of the non-linear power flow constraints, when solved to optimality, provide valid bounds to the original problem because their feasible sets include all the solutions of the original problem. Convex relaxations are especially useful because their solutions are globally optimal for the relaxed problem, and the cuts generated by these relaxations are valid outer approximations for the real problem. However, as outer approximations, these cuts might lead to optimistic solutions. Although many convex relaxations exist for the optimal power flow problem, we focus on a limited subset. One simple linear relaxation used in the Brazilian official dispatch tools is the NFA, in which power flow limits are considered for each line, but KVL is ignored. 
%
In this lossless model, all the energy that is injected from an arbitrary bus $n$ into a line $(n,m)$, outputs at the receiving bus $m$. In other words, we make $\mathcal{X}_t \leftarrow \mathcal{X}_{NFA,t}$ in \eqref{OPF} where:
\begin{subequations} \label{NFA_PF}
    \begin{align}
        \mathcal{X}_{NFA,t} = \Big\{ \mathbf{x}_t \Big\vert \, f_{(n,m)t} = - f_{(m,n)t}\;\; \forall (n,m) \in \mathcal{L}\Big\}
    \end{align}
\end{subequations}

One of the more sophisticated convex relaxations is the \textit{semidefinite programming relaxation} (SDP). This formulation is obtained by replacing \eqref{eq_ac_w} by $\mathbf{W}_t \succeq 0 \land rank(\mathbf{W}_t)=1$ and then dropping the rank constraint, that is where all the non-convexity lies \cite{BAI2008383}. Hence, we define:
\begin{subequations} \label{SDP_PF}
    \begin{align}
        %
        \mathcal{X}_{SDP,t}= \Big\{ \mathbf{x}_t  \Big\vert \, \exists \; q_t,\mathbf{W}_t,f^q_t : \text{\eqref{eq_voltage_acw_bounds}--\eqref{eq_gen_q_bounds_acw}}, \mathbf{W}_t \succeq 0  \Big\} .
    \end{align}
\end{subequations}

The \textit{Second-Order Cone relaxation} (SOC) is a non-linear convex relaxation that is tighter than NFA, but looser than SDP, \cite{1664986}. The feasible region of the AC formulation, shown in \eqref{AC_W_PF}, is contained within the feasible region of the SDP relaxation \eqref{SDP_PF}, which is contained in the SOC set \cite{low2014convex,low2014convex2}.
This time, \eqref{eq_ac_w} is replaced by: $|\mathrm{w}_{nmt}|^2 \leq  |v_{nt}|^2|v_{mt}|^2 = \mathrm{w}_{nnt}\mathrm{w}_{mmt}$.
The resulting problem may be specified as a second-order cone formulation, shown in \eqref{SOC_PF}.

$\mathcal{X}_{SOC,t} = \Big\{ \mathbf{x}_t \Big\vert \, \exists \; q_t,\mathbf{W}_t,f^q_t$: \eqref{eq_voltage_acw_bounds}--\eqref{eq_gen_q_bounds_acw},
\begin{subequations} \label{SOC_PF}
    \begin{align}
        %
        & |\mathrm{w}_{nmt}|^2 \leq  \mathrm{w}_{nnt}\mathrm{w}_{mmt} \;\; \forall(n,m) \in \mathcal{L} \Big\} .
    \end{align}
\end{subequations}

Instead of relaxing, it is possible to approximate the non-linear Kirchhoff's Voltage Law equations through $\mathcal{X}_{DC,t}$, a linear DC power flow \cite{Stott2009_DC}. Alternatively, $\mathcal{X}_{DC,t}$ can be used to consider the quadratic DCLL approximation, which provides more accurate results \cite{coffrin2012approximating}, and can also be implemented through piecewise linear approximations. Both implementations are standard in power system and for the sake of brevity are omitted. We refer to \cite{Coffrin2018PowerModels} for the practical implementations of these models.

\begin{comment}

    Instead of relaxing, it is possible to approximate some of the non-linear power flow constraints. The \textit{linear DC approximation} (DC) \cite{Stott2009_DC} is a linear formulation, which partially represents power voltages. Some assumptions are made to achieve such formulation: voltage magnitudes are close to the nominal value, angle differences are close to zero, and line power losses are negligible.
    Following these assumptions the DC power-flow set $\mathcal{X}_{DC,t}$ can be defined as follows:
    %
    \begin{subequations} \label{DC_PF}
        \begin{align}
            & \mathcal{X}_{DC,t} = \Big\{ \mathbf{x}_t \Big\vert \, \exists \; \theta_{t} : \ell_{nt} = 0 \;\; \forall n \in \mathcal{N} \label{eq_loss_DC}\\
            %
            & f_{(n,m)t} = -\left(B_{(n,m)t}\right) (\theta_{nt} - \theta_{mt})\;\; \forall (n,m) \in \mathcal{L} \label{eq_power_DC}\\
            & f_{(m,n)t} = -\left(B_{(n,m)t}\right) (\theta_{mt} - \theta_{nt})\;\; \forall (n,m) \in \mathcal{L} \label{eq_power_DC_2} \Big\}
        \end{align}
    \end{subequations}
    where $B_{(n,m)t} = ({X_{(n,m)t})^{-1}}$.
    
    Still, it is important to notice that, while this model approximates the feasible region of the AC power flow, it might not include the entire feasible region. Therefore, the global optimum of the AC optimal power flow problem can be lost. It is worth mentioning that this approximation is not guaranteed to be optimistic  (like the convex relaxations) nor pessimistic.
    
    One extension of the DC model is the \textit{DCLL approximation}, see \cite{coffrin2012approximating} for more details. 
    To do that, the equality is replaced with an inequality, i.e., $f_{(n,m)t} + f_{(m,n)t} \ge $ line losses.
    It will be defined as follows:
    %
    
    ORIGINAL
    
    \begin{subequations} \label{DCLL_PF}
        \begin{align}
            & \mathcal{X}_{DCLL,t}= \Big\{ \mathbf{x}_t \Big\vert \, \exists \; \theta_t : \ell_{nt} = 0 \;\; \forall n \in \mathcal{N}, \label{eq_loss_DCLL_bus}\\
            %
            & f_{(n,m)t} = -\left(B_{(n,m)t}\right) (\theta_{nt} - \theta_{mt})\;\; \forall (n,m) \in \mathcal{L} \label{eq_power_DCLL}\\
            & f_{(n,m)t} + f_{(m,n)t} \geq 
            \frac{G_{(n,m)t}}{G_{(n,m)t}^2 + B_{(n,m)t}^2}f_{(n,m)t}^2\;\; \forall (n,m) \in \mathcal{L} \Big\}, \label{eq_loss_DCLL}
        \end{align}
    \end{subequations}
    
    % TESTE JG
    
    % \begin{subequations} \label{DCLL_PF}
    %     \begin{align}
    %         & \mathcal{X}_{DCLL,t}= \Big\{ \mathbf{x}_t \Big\vert \, \exists \; \theta_t : , \label{eq_loss_DCLL_bus}\\
    %         %
    %         & f_{(n,m)t} = -\left(B_{(n,m)t}\right) (\theta_{nt} - \theta_{mt})\;\; \forall (n,m) \in \mathcal{L} \label{eq_power_DCLL}\\
    %         & \ell_{nt} \geq \frac{1}{2} R_{(n,m)t} f_{(n,m)t}^2 \;\; \forall (n,m) \in \mathcal{L} \Big\}, \label{eq_loss_DCLL}
    %     \end{align}
    % \end{subequations}

\end{comment}

\subsection{Open-source Julia package: HydroPowerModels.jl}

Solving a hydrothermal dispatch problem depends on the complex and not always easily available SDDP algorithm. 
However, until recently, there was no fast, reliable, and open-source implementation of the SDDP algorithm. Without such a tool, researchers and practitioners have not had a common ground for discussing and analyzing different hydrothermal dispatch formulations and their solutions. Together with this work we made available an open-source tool, called \href{https://github.com/andrewrosemberg/HydroPowerModels.jl}{\textit{HydroPowerModels.jl}} \cite{Rosemberg2020}, that can be this common ground. \textit{HydroPowerModels.jl} can be used to assess the impact of modeling choices during the planning of a hydrothermal power system, as we show in the next section.


==> Sec-TBackground.tex <==
The goal of the hydrothermal economic dispatch problem is to find the optimal operation policy of an electrical system to meet demand throughout a long-run planning horizon. For this purpose, the policy must take into account the best use of water to ensure power balance across the network during all periods under the uncertainty of inflows, demand, fuel costs, etc. We will consider only the inflow uncertainty to avoid deviating from our main focus. The HTD is modeled as a large-scale multistage stochastic optimization problem and generally solved by SDDP \cite{pereira1991multi,philpott2013solving,dowson_sddp.jl}. 

The complete mathematical formulation of the HTD in one stage, will be represented by the function $\mathcal{Q}_t(\nu_{t-1},\omega_t) =$
\begin{subequations} \label{OPF}
    \begin{align}
        %
        \hspace{-1cm}\underset{\mathbf{x}_t}{\mbox{min: }} & \sum_{i \in \mathcal{I}} C_{it} \, p_{it} + \sum_{n \in \mathcal{N}} C^{\delta}_{nt} \, \delta_{nt} + \mathbb{E}[\mathcal{Q}_{t+1}(\nu_{t}, \omega_{t+1})] \label{eq_objective}\\
        %  + \sum_{j \in \mathcal{H}} C^{s}_{jt} \, s_j
        \mbox{s.t.: } & \nonumber \\
        & \sum_{\substack{i \in I_n}} p_{it} + \sum_{\substack{j \in \mathcal{H}_n}} u_{jt} \, \rho_{jt} -\sum_{\substack{m \in \mathcal{N}_n}} f_{(n,m)t} - \ell_{nt} + \nonumber \\
        & \qquad  =  D_{nt} - \delta_{nt}, \;\; \forall n\in \mathcal{N} \label{eq_kcl_shunt} \\
        & \nu_{jt} + u_{jt} + s_{jt} = \nu_{j,t-1} + A_{j,t}(\omega_t) + \nonumber \\ 
        & \qquad  \sum_{\substack{k \in \mathcal{H}^U_j}} u_{kt} + \sum_{\substack{k \in \mathcal{H}^{S}_j}} s_{kt}, \;\; \forall j \in \mathcal{H} \label{eq_hydro_balance} \\
        & |f_{(n,m)t}| \leq F_{(n,m)t},\; |f_{(m,n)t}| \leq F_{(n,m)t} \;\; \forall (n,m) \in \mathcal{L} \label{eq_thermal_limit}\\
        % & |f_{(m,n)t}| \leq F_{(n,m)t} \;\; \forall (n,m) \in \mathcal{L} \label{eq_thermal_limit_2}\\
        & 0 \leq p_{it} \leq P_{it} \;\; \forall i \in I  \label{eq_gen_bounds}\\
        & 0 \leq \nu_{jt} \leq \overline{\nu}_{jt} \;\; \forall j \in \mathcal{H} \label{eq_volume_limit}\\
        & 0 \leq u_{jt} \leq U_{jt} \;\; \forall j \in \mathcal{H} \label{eq_outflow_limit} \\
        %& \mathbf{x}_t \in \mathbf{Proj}_{\mathbf{x}_t} \left(\mathcal{X}_t \right). \label{eq_XT}
        & \ell_{nt} \geq 0 \;\; \forall n \in \mathcal{N} \label{eq_loss_opf} \\
        & \delta_{nt} \geq 0 \;\; \forall n \in \mathcal{N} \label{eq_def_opf} \\
        & \mathbf{x}_t \in \mathcal{X}_t. \label{eq_XT}
    \end{align}
\end{subequations}
%
$\mathbf{x}_t$ is the stacked vector of all decision variables, $\mathbf{x}_t = [p_t, f_t, u_t, s_t, \nu_t, \delta_t, \ell_t]^T$, and $\mathcal{X}_t$ represents different power-flow constraints related to the associated network formulation. 

The objective function \eqref{eq_objective} is to minimize the sum of immediate costs represented by the costs of active power generation and the cost of energy supply deficit, and future costs represented by the cost-to-go function $\mathbb{E}[\mathcal{Q}_{t+1}(\nu_{t}, \omega_{t+1})]$.
Constraints \eqref{eq_kcl_shunt} implements Kirchhoff’s Current Law (KCL), i.e., power balance at each node. Deficit variables guarantee feasibility in case of a lack of power availability.
The water mass balance equation is implemented in \eqref{eq_hydro_balance}, where the water stored in a reservoir should equal the water previously stored plus the incoming inflows and water discharged from upstream reservoirs, minus the portion used to generate energy and the one spilled away.
Constraints \eqref{eq_thermal_limit} to \eqref{eq_def_opf} represent physical limits on variables.
Finally, expression \eqref{eq_XT} represents a feasibility set used to model all network models considered in this work. The characterization of this set to represent the different network models is made in section \ref{sec:pf}.

Simplified Optimal Power Flow (OPF) network formulations, $\mathcal{X}_t$, are a necessary condition to achieve a tractable model that is also compatible with efficient solution methods such as SDDP. Planning agents use simplified models to find the best reservoir levels in medium- and long-term horizons by computing the cost-to-go functions. For implementing operating decisions, however, independent systems operators (ISO) seek feasible dispatches complying with more detailed network models. This is done by coupling the simplified view of the systems' future operation, implicitly considered in the cost-to-go function, with more realistic network formulations. Unfortunately, in practice, the simplifications considered in the network model to evaluate cost-to-go functions are significantly optimistic compared to the representation needed to ensure feasibility. This optimistic bias leads to the implementation of expensive (sub-optimal) time-inconsistent policies \cite{7859406}.

For instance, in the Brazilian case, where ISOs apply the SDDP algorithm using the NFA model representation to estimate the cost-to-go function used as input in a second model with a more accurate representation of the network. Then, in the next period, the state is updated with the actual reservoir levels and the same process is repeated. In Chile, conversely, SDDP is implemented with a DC with losses model, and this may vary from system to system according to the perception of the impact each representation may bring. This rolling-horizon operating scheme produces a time-inconsistent policy in which implemented decisions deviate from those obtained in the planning stage embedded in the cost-to-go function. Hence, this hybrid and inconsistent implemented policy deliver decisions that can be far from optimal, both for the planning problem and for the true optimal policy fully based on the detailed model. 

To evaluate the performance of the time-inconsistent policies induced by network simplifications, we follow the framework proposed in \cite{7859406}. According to the previously described decision process, two different models for the network are used: $\mathcal{X}_t^{plan}$ on the planning stage, where the cost-to-go functions are estimated in the backward pass, and $\mathcal{X}_t^{imp}$ when simulating the actually implemented dispatch decisions. Aiming to isolate the effect of a given network model, the difference between the planning model and the implementation model, in this work, is defined by which model is considered in $\mathcal{X}_t$. In this context, it is worth mentioning that the only result of the planning stage used in the implementation phase of period $t$ is the cost-to-go function, $\mathbb{E}[\mathcal{Q}_{t+1}^{plan}]$, which represents the opportunity cost of the water. We refer to \cite{AndrewThesis} for further details on the estimation and simulation procedure using the two different models.

To quantify the time-inconsistency gap, i.e. the modeling risk, we compare the cost of the actual implemented inconsistent policy, $\mathcal{P} \big(\{\mathcal{Q}_t^{plan}\}^T_{t=1}, \{\mathcal{X}_t^{imp}\}^T_{t=1}, \{\omega_{t,s}\}^{T,M}_{t=1,s=1} \big)$, with the cost of the respective reference planning policy, $\mathcal{P} \big(\{\mathcal{Q}_t^{plan}\}^T_{t=1}, \{\mathcal{X}_t^{plan}\}^T_{t=1}, \{\omega_{t,s}\}^{T,M}_{t=1,s=1} \big)$. $\mathcal{P}$ represents all the simulation results for a policy using a given set of cost-to-go functions, a given set describing the network model, and a given set of inflow scenarios.
Hence, the time-inconsistency gap measures the hidden cost of neglecting the constraints of the implementation problem in the planning phase. It can be seen as the operator's regret with respect to its planning expectations. Consequently, it allows ISOs to detect and quantify the impact of the inconsistencies induced by a given simplification without the need of simulating the full, and possibly currently intractable, policy based on the more complex network model such as the AC power flow.


